High-dimensional Filtering using Nested Sequential Monte Carlo

Sequential Monte Carlo (SMC) methods comprise one of the most successful approaches to approximate Bayesian filtering. However, SMC without good proposal distributions struggle in high dimensions. We propose nested sequential Monte Carlo (NSMC), a methodology that generalises the SMC framework by requiring only approximate, properly weighted, samples from the SMC proposal distribution, while still resulting in a correct SMC algorithm. This way we can exactly approximate the locally optimal proposal, and extend the class of models for which we can perform efficient inference using SMC. We show improved accuracy over other state-of-the-art methods on several spatio-temporal state space models.

==> sec-background.tex <==
\begin{itemize}
\item Introduce nested importance sampling
\item Proper weighting and random weights
\item Introduce \smc to generate pws
\item Backward simulation to generate pws
\item Theory
\begin{itemize}
\item Proper weighting of Nested IS
\item Proper weighting of SMC
\item Asymptotic variance of Nested IS with internal IS and SMC on independent example? (nice results on how we get exact sampler in $M \to \infty$)
\end{itemize}
\end{itemize}
% ======================================================================
%                           NESTED IS
% ======================================================================
\section{Nested Importance Sampling}\label{sec:background}
A special case of the novel family of methods we introduce in this paper is the slightly more straightforward nested importance sampling (\nis) method. We will use this method to lay the groundwork and introduce some of the more fundamental concepts used to construct the fully general nested \smc family of methods in the next section. Typically in importance sampling we are interested in approximating intractable expectations of a function $\varphi$ with respect to some \emph{target distribution} of interest $\pi(x)$ 
\begin{align}
\pi(\varphi) \eqdef \E_\pi[\varphi(X)] = \int \varphi(x) \pi(x) \myd x.\label{eq:is:expectation}
\end{align}
Furthermore, we might only know $\pi(x)$ up to some multiplicative constant, \ie
\begin{align}
\pi(x) = \frac{1}{Z_\pi} \gamma(x),\label{eq:is:target}
\end{align}
where $\gamma(x)$ is the unnormalised target distribution and $Z_\pi \eqdef \int \gamma(x) \myd x$ the constant ensuring that $\pi(x)$ is a proper probabilistic density function (\pdf). The importance sampling method is obtained by generating some set of \iid weighted samples (or particles) $\{\left(X^i,W^i\right)\}_{i=1}^N$ such that the estimator of \eqref{eq:is:expectation}, given by
\begin{align}
\pi(\varphi) \approx \sum_{i=1}^N \frac{W^i}{\sum_\ell W^\ell} \varphi(X^i),\label{eq:is:approx:expectation}
\end{align}
approaches the correct one $\pi(\varphi)$ in the limit of infinite number of samples. The intuition in \nis will be to make use of structure in $\gamma(x)$ and then use internal \is or \smc-algorithms to generate the samples $(X^i, W^i)$. But before we introduce \nis we will study some of the fundamental concepts that makes \is work.


% ======================================================================
%                      PROPER/RANDOM WEIGHTS
% ======================================================================
\subsection{Proper and Random Weights in Importance Sampling}
Typically \is uses a given proposal $q(x)$ to draw \iid samples and the weights are then defined by $w(x) = \frac{\gamma(x)}{q(x)}$. However, it is possible to replace the standard deterministic (conditional on sampled $x$) \is weight by an unbiased estimate of it and still obtain a consistent estimate \citep[p. 37]{liu2001monte}. More precisely $W$ is a random variable where the conditional expectation $\E[W | X = x] \propto w(x)$, and we refer to this method as a \emph{random weights} IS (\rwis) method. If the random weights are also non-negative, \ie $W\geq 0$ almost surely, then we can motivate this approach by considering $W$ to be an auxiliary variable and extend the target distribution accordingly. The way we prove correctness of \nis and \nsmc will be of a similar flavour, \ie constructing an extended target and show that the algorithms are standard \is or \smc methods for these extended targets. Furthermore, we will also make use of the following key property.
\begin{definition}[Properly weighted sample]
The (random) pair $(X,W)$ is a \emph{properly weighted sample} for a distribution $p(x)$ if $W \geq 0$ and ${\E[W\varphi(X)] = D p(\varphi)} = D \int \varphi(x) p(x) \myd x$, for all measurable functions $\varphi$ and some constant $D \in \reals_+$.
\end{definition}
Note that the requirements on $(X,W)$ given by the definition of a properly weighted sample is in fact equivalent to the one of the (non-negative) random weights \is above.

Now, interestingly, it is sufficient to generate samples properly weighted \wrt the \emph{proposal} $q(\cdot)$ to construct a valid \is algorithm. Typically, in the \is case we will be interested in choosing $q = \pi$ and construct an efficient \emph{nested} (or inner) algorithm to generate properly weighted samples from it. Formally, we assume that we can not simulate exactly from $q$ but we can evaluate its unnormalized density $r(x) \eqdef Z_q q(x)$. Furthermore, assume we have access to some distribution $Q_M(x,z)$ on the product space of $(x,z) \in \setX \times \reals_+$ that generates \iid samples $(X^i,\hat Z_q^i)$ properly weighted with respect to $q$. The distribution is indexed by $M$ to highlight the fact that we will use nested \is (and \smc) to construct $Q_M$. With this notation in place it is now possible to define the nested importance sampler, see Algorithm~\ref{alg:nis}.
\begin{algorithm}
\caption{Nested Importance Sampling \hfill (steps 1--2 for $i=1,\ldots,N$)}\label{alg:nis}
\begin{algorithmic}[1]
\STATE Simulate $(X^i, \hat Z_q^i) \iidsim Q_M(x,z)$
\STATE Set weights $W^i = \frac{\hat Z_q^i \pi(X^i)}{r(X^i)}$
\STATE Compute $\hat Z_\pi = \frac{1}{N}\sum_{i=1}^N W^i$ 
\end{algorithmic}
\end{algorithm}

% ======================================================================
%                               SMC
% ======================================================================
\subsection{Sequential Monte Carlo}


% ======================================================================
%                               BS
% ======================================================================
\subsection{Backward Simulation}

